Towards a Theory of Control Architecture: A quantitative framework for layered multi-rate control

This paper focuses on the need for a rigorous theory of layered control architectures (LCAs) for complex engineered and natural systems, such as power systems, communication networks, autonomous robotics, bacteria, and human sensorimotor control. All deliver extraordinary capabilities, but they lack a coherent theory of analysis and design, partly due to the diverse domains across which LCAs can be found. In contrast, there is a core universal set of control concepts and theory that applies very broadly and accommodates necessary domain-specific specializations. However, control methods are typically used only to design algorithms in components within a larger system designed by others, typically with minimal or no theory. This points towards a need for natural but large extensions of robust performance from control to the full decision and control stack. It is encouraging that the successes of extant architectures from bacteria to the Internet are due to strikingly universal mechanisms and design patterns. This is largely due to convergent evolution by natural selection and not intelligent design, particularly when compared with the sophisticated design of components. Our aim here is to describe the universals of architecture and sketch tentative paths towards a useful design theory.

==> formatting.tex <==
\section{Formatting}
In assembling the main text, pay careful attention to the order of topics as well as the sectioning. Choose section and subsection headings to reflect the material and serve as a road map for the reader. Do not provide a section heading at the beginning of your article, which \textit{IEEE CS} assumes is the introduction. You can use subsubsection headings if you wish, but be sure to use them carefully so the reader can follow the layout. Please use this style for review purposes:

\begin{itemize}
\item Section heads: Centered, bold, large font \verb|\section{}|

\item Subsection headings: Left justified, bold, regular size font \verb|\subsection{}|

\item Subsubsection headings: Left justified, not bold, regular size font, italics \verb|\subsubsection{}|

\end{itemize}

\noindent An example can be treated as a subsection or subsubsection.

\subsection{Figures, Tables, and Captions}

\textit{IEEE CS} requires a uniform style for figure and table captions that is intended to enhance the quality and appearance of articles. Be sure that every figure and table is well motivated and transmits an essential point in relation to the main ideas of the article. \textit{IEEE CS} uses a descriptive and informative style for figure and table captions that enhances the impact and appeal of figures. You can think of a figure or table caption as a summary of what you would say if you were presenting the figure or table in a PowerPoint presentation.

Each caption must be informative, interesting, and helpful. The figure or table caption may provide a summary of the main points from the text. In fact, repetition between the figure caption and text is encouraged. A figure or table caption can also be used as a mini tutorial for the reader. These captions will greatly enhance your article and the overall quality of \textit{IEEE CS}.

The general style is that the figure should not have a caption or label along the top. The axes are labeled, and a legend should be used. Multiple curves can be distinguished by color or dashes and dots. The caption below the figure includes a title and one or more sentences of pertinent information.

\begin{itemize}
\item Avoid using acronyms in figures and figure captions so that the figure captions can be read independently of the text. If an acronym appears in a figure, then please redefine the acronym in the figure caption.  

\item Please be sure that every figure, table, and sidebar is cited in the main text. 

\item Table captions should be equally informative and located above the table, as shown in Table \ref{tab1}.

\end{itemize}

It is the responsibility of the author to obtain copyright permission for all materials that are subject to copyright protection. It is the author's responsibility to obtain this permission prior to final acceptance of the manuscript. You do not need to obtain copyright permission before you submit your article. Each relevant figure caption must include an explicit statement that permission has been given. At the end of the figure caption, include a statement such as ``(With permission of Smith and Jones Publishers.)'' or ``(Image courtesy of Technocontrol, Inc.).''

The suggested caption format is (see Figure \ref{fig1}):

\begin{figure}[b]
\centerline{\includegraphics[width=18.0pc]{fig1.eps}}
\caption{An example of a figure.  This text does not have any relation to the figure itself. (Courtesy of XYZ. Company.)\label{fig1}}
\end{figure}

\noindent\looseness=-1FIGURE 1 Title of the plot, not a sentence. Next, a sentence is given here to indicate the points that the figure is meant to highlight. Finally, you can include additional sentences to provide more detail about the meaning and importance of the figure. These sentences will greatly enhance the appeal of your article. (With the permission of Bodeplots, Inc.)

\subsection{References}

All cited references must be publicly accessible. Internal reports, theses, and dissertations are not viewed as being publicly accessible and, thus, cannot be included in the reference list. \textit{IEEE CS} is an archival publication, whose articles are backed up by other archival publications.  However, obscure or unpublished documents that can be accessed from the web can be cited as long as the citation includes a URL address from which the document can be accessed. In these cases, a website must be provided from which the document can be obtained. All references need to be complete and accurately state the authors, title, volume, pages, and date. 

\subsubsection{Citation Style in the Text}

References must be listed in the order of citation in the text.  Reference citations in the text must be bracketed numbers, that is, [3]--[5], [23]. For multiple nonsequential citations, separately bracket each number in numerical order, that is, [3], [5], [7]. In \LaTeX{}, the package \verb|\usepackage[compress]{cite}| can be used to produce the required style.

Avoid mentioning authors by names in the text. It is acceptable to mention illustrious names such as Newton and Bode, but please do not mention the names of contemporaries. The passive voice is fine.

\begin{itemize}

\item Do not write ``Jones [22] shows that...,'' instead write ``It is shown in [22] that...''

\item Do not put http:// addresses in the text. Rather, put all web addresses in the reference list as separate items.
\end{itemize}

\subsubsection{Bibliography Style and Guidelines}

The preferred style is listed below, but it is acceptable to use the standard IEEE bibstyle file \cite{BB1}.

\begin{itemize}

\item Do not include private communications in the reference list. The acknowledgments can be used for this purpose.

\item Do not include full first names of authors, only initials. Initials come first; that is, F. G. Smith.

\item Do not use ``et al.'' Instead, always list all authors.

\item For the title of an article, capitalize only the first word, and place the title in quotes.

\item The names of journals and proceedings are italicized.

\item Location is included for conferences.

\item For journal articles, include vol. and no., lower case and abbreviated in each case, and set  off with commas.

\item Page numbers appear after the year of publication for conference proceedings and books, but before the year of publication for journals.

\item For documents available online, cite the location and date last accessed.

\end{itemize}

\noindent Examples:

\noindent [1] A. Smith, B. Jones, and J. Doe, ``Control technology,'' in \textit{Proc. 123rd Conf. on Control}, Anchorage, AK, 1999, pp. 123--234.

\noindent [2] A. Smith, B. Jones, and J. Doe, ``Control technology,'' \textit{Trans. Contr.}, vol. 1, no. 1, pp.  123--234, 1999.

\noindent [3] A. Smith, B. Jones, and J. Doe, ``Control technology,'' in \textit{Control Tech.}, I.M. Aneditor, Ed. Boston: Minuteman Press, 1999, pp. 123--234.

\noindent [4] R. P. Bemis, Ed., \textit{Control Technology}. Holyoke: Hillview Press, 1999.

\noindent [5] W. Burke, \textit{Control in Extreme Climates}. Minneapolis, MN: Environmental Press, 1999.

\noindent [6] A. Smith. \textit{The Dictionary} (10th ed.) Available online at http://www.thedictionary.com  (last accessed May, 2016).

\noindent [7] A. Smith, ``Control technology,'' \textit{IEEE Trans. on Control Systems Technology}, vol. 20, no. 2, pp. 5--10, June 2000.

\noindent [8] ``Advances in Estimation.'' Available online at http://www.filtermethods.com (last accessed May, 2016).

\subsection{Sidebars}

A sidebar is a self-contained digression that provides additional information in support of the main text. Sidebars are strongly encouraged since readers find these digressions useful and informative. See ``Sidebars In \textit{IEEE Control Systems}'' for more information.

\subsection{Author Biographies}

At the end of your article, please include a brief biography of every author. Do not include  place or date of birth. Include details of education. Say ``the B.S. degree,'' not ``his B.S. degree.'' Mention the name of each author only once in each biography. Do not use bold font for authors' names. Limit biographies to 200 words. Do not include photos in your article; they will be requested at a later date. Include the email and mailing address of only the corresponding  author.

\section{Writing Styles}

In preparing your article for \textit{IEEE CS}, please note the following guidelines concerning writing style. \textit{IEEE CS} places high emphasis on the quality and precision of exposition. Articles that are not well written cannot be considered for publication. Many of the guidelines below reflect standard writing practice. However, a few of these guidelines are specific to \textit{IEEE CS}.

\subsection{Tone of Writing}

Adopt an objective, scientific tone. It is acceptable to use ``we'' sparingly. Please avoid the  vague subject ``one.'' Passive voice is fine and preferable to ``one.'' Do not refer to the reader as ``you.'' Along the same lines, do not use the word ``our.'' Your article is a scientific essay, not a  report on what your group possesses. Be objectively and dispassionately descriptive in referring to ``the testbed'' rather than ``our testbed.'' Refer to your work in the same objective style that you refer to the work of other researchers.

\begin{sidebar}{Sidebars in {\it IEEE Control Systems}}

\setcounter{sequation}{0}
\renewcommand{\thesequation}{S\arabic{sequation}}
\setcounter{stable}{0}
\renewcommand{\thestable}{S\arabic{stable}}
\setcounter{sfigure}{0}
\renewcommand{\thesfigure}{S\arabic{sfigure}}

\sdbarinitial{A} sidebar is a self-contained digression that provides additional information in support of  the main text. Sidebars are strongly encouraged since readers find these digressions useful and informative. Place sidebars at the end of the document, starting each one on a new page. Every sidebar must be mentioned in the main text using the style `For details, see ``How Does Fusion Work?''' The technique for referencing sidebars in the main body of the text is as follows. The  sidebar title is created using the command

\begin{verbatim}\section[How Does Fusion Work?]{Sidebar: 
   How Does Fusion Work?} \label{sidebar-HDFW}.\end{verbatim}

The text might then include a sentence such as, `See ``\verb|\nameref{sidebar-HDFW}|'' for more details on techniques that can be used to increase the controller robustness.' You will need to add \verb|\usepackage[draft]{hyperref}| for this to work.

\sdbarfig{\includegraphics[width=19.0pc]{fig1.eps}}{Note that figures in sidebars are numbered as S1, S2, and so on, to distinguish them from ones in the main text of the article.\label{sfig1}}

Figures and tables in sidebars are numbered as Figure \ref{sfig1} and Table \ref{stab1}. If the first sidebar has Figure \ref{sfig1} and Figure S2, then the first figure in the second sidebar is numbered S3. The same numbering scheme is used for equations and tables that appear in sidebars. To manually label sidebar equations in LaTeX, use \verb|tag*{\mbox{\rm{S4}}}|. Sidebar equations and figures  can be automatically numbered by using the commands listed below.

\bgroup{\fontsize{7.5pt}{12pt}\selectfont\begin{verbatim}
\setcounter{sequation}{0}
\renewcommand{\thesequation}{S\arabic{sequation}}
\setcounter{stable}{0}
\renewcommand{\thestable}{S\arabic{stable}}
\setcounter{sfigure}{0}
\renewcommand{\thesfigure}{S\arabic{sfigure}}
\end{verbatim}}\egroup

\sdbartable{Units for magnetic
properties.\label{stab1}}{\begin{tabular*}{18.5pc}{@{}|p{27pt}|p{67pt}<{\raggedright}|p{90pt}<{\raggedright}|@{}}
\hline
&  & \textbf{Conversion from} \\
&  & \textbf{Gaussian and  CGS} \\
\textbf{Symbol} & \textbf{Quantity} & \textbf{EMU to SI}$^{\mathrm{a}}$ \\
\hline
$\Phi $& 
Magnetic flux& 
1 Mx $\to  10^{-8}$ Wb $= 10^{-8}$ V $\cdot$ s \\
$B$& 
Magnetic flux density,   magnetic induction& 
1 G $\to  10^{-4}$ T $=$\break $10^{-4}$ Wb/m$^{2}$ \\
$H$& 
Magnetic field strength& 
1 Oe $\to  10^{-3}/(4\pi )$ A/m \\
$m$& 
Magnetic moment& 
1 erg/G $=$ 1 emu   $\to$\break $10^{-3}$ A $\cdot$ m$^{2} = 10^{-3}$ J/T \\
$M$& 
Magnetization& 
1 erg/(G $\cdot$ cm$^{3}) =$\break 1 emu/cm$^{3}$   $\to 10^{-3}$ A/m \\
\hline
\end{tabular*}}

A sidebar can cite references from the bibliography of the main text or it can have its own bibliography using the numbering style [S1], [S2]. The same scheme is used for sidebar figures and tables. See the ``Use of References in a Sidebar'' section for further details. Sidebar references can be  manually numbered as follows.

\begin{verbatim}
\begin{thebibliography}{99}
\bibitem[S7]{Kailath} T. Kailath, {\em Linear 
   Systems}, Prentice Hall, 1980.
\bibitem[S8]{Courant} R. Courant and D. Hilbert, 
   {\em Methods of Mathematical Physics}, 
   Interscience, 1953.
\end{thebibliography}
\end{verbatim}

Sidebar references can also be automatically numbered using these steps:

\begin{enumerate}

\item Place each part of the article that is to have a separate bibliography in an include file, with \verb|\bibliography| as the last line.

\item Add \verb|\usepackage{chapterbib}| in the main latex file.

\item Run latex and bibtex as usual.

\item Comment out the \verb|\usepackage{chapterbib}| and all \verb|\bibliography| and \verb|\bibliographystyle| commands.

\item Copy the .bbl files into the main latex file.

\item Run latex and comment out duplicate \verb|\bibitem| entries in the sidebar bibliographies.

\item Relabel the references in the sidebars as \verb|\bibitem[S1]{...}|.

\end{enumerate}

\section{Sidebar level heading}

Sidebars must be cited in the text. The sidebars will be placed in the the text in the order in which they are mentioned. Note that all figures and tables in sidebars must also be cited in numerical order in the sidebar. 

\end{sidebar}

\begin{sidebar}{\continuesidebar}

\setcounter{sequation}{0}
\renewcommand{\thesequation}{S\arabic{sequation}}
\setcounter{stable}{0}
\renewcommand{\thestable}{S\arabic{stable}}
\setcounter{sfigure}{0}
\renewcommand{\thesfigure}{S\arabic{sfigure}}

\subsection{Sidebar Sub Level Head}

Equation numbers in a sidebar start with S, the same as figures and tables. Equation numbers must be sequential. Equation numbering can be continued from one sidebar to another. For example, if the last equation number in this sidebar is (S10), the first numbered equation in the next sidebar would be (S11).

\subsection{Use of References in a Sidebar}

Here is some random text showing how references are handled for a sidebar. Reference \cite{SAA1} gives one random reference. A basic equation is
\begin{sequation}
f = ma,\label{seq1}
\end{sequation}
and the impact of \eqref{seq1} is highlighted in Figure \ref{sfig1}. Reference \cite{SAA2} gives another random reference, but \cite{AA1} and \cite{BB1} are references in the main body of the text that can be cited in the sidebar.

\begin{thebibliography}{S1}
\bibitem[S1]{SAA1}
T. E. Passenbrunner, M. Sassano, M. Hirsch, and L. del Re,
``Identification and inverse torque control of hydrodynamic
dynamometers,'' \textit{IEEE Trans. Control Syst. Technol.}, vol. 22, no. 2,
pp. 607--617, Mar. 
2014. doi: 10.1109/TCST.2013.2262531.

\bibitem[S2]{SAA2}
M. Hirsch and T. E. Passenbrunner, ``Extension of static non-linear
DOE identification algorithms to dynamic systems,'' in \textit{Computer
Aided Systems Theory}, R. Moreno-D\'{i}az, F. Pichler, A.
Quesada-Arencibia, Eds. Berlin: Springer-Verlag, 2011, pp. 33--40.

\end{thebibliography}

\end{sidebar}

\setcounter{equation}{0}

A historical overview can appear in the introduction or a sidebar.  However, reportorial writing in describing the technical results is not allowed. Do not describe how you developed your results or how and why your research progressed. In fact, experimental or computational results can usually be described as if they are unfolding in the present with an objective description. Your article must not be written as a report of your past activities; see the section ``Tense.''

\begin{table}
\caption{Units for magnetic properties.\label{tab1}}
\begin{tabular*}{18.5pc}{@{}|p{29pt}|p{69pt}<{\raggedright}|p{86pt}<{\raggedright}|@{}}
\hline
& & Conversion from \\
& & Gaussian and  CGS \\
Symbol& Quantity& EMU to SI$^{\mathrm{a}}$ \\
\hline
$\Phi $& 
Magnetic flux& 
1 Mx $\to  10^{-8}$ Wb $= 10^{-8}$ V $\cdot$ s \\
$B$& 
Magnetic flux density,   magnetic induction& 
1 G $\to  10^{-4}$ T $= 10^{-4}$ Wb/m$^{2}$ \\
$H$& 
Magnetic field strength& 
1 Oe $\to  10^{-3}/(4\pi )$ A/m \\
$m$& 
Magnetic moment& 
1 erg/G $=$ 1 emu   $\to 10^{-3}$ A $\cdot$ m$^{2} = 10^{-3}$ J/T \\
$M$& 
Magnetization& 
1 erg/(G $\cdot$ cm$^{3}) =$ 1 emu/cm$^{3}$   $\to 10^{-3}$ A/m \\
4$\pi M$& 
Magnetization& 
1 G $\to  10^{-3}/(4\pi )$ A/m \\
$\sigma $& 
Specific magnetization& 
1 erg/(G $\cdot$ g) $=$ 1 emu/g $\to $ 1 A $\cdot$ m$^{2}$/kg \\
$j$& 
Magnetic dipole   moment& 
1 erg/G $=$ 1 emu   $\to 4\pi \times  10^{-10}$ Wb $\cdot$ m \\
$J$& 
Magnetic polarization& 
1 erg/(G $\cdot$ cm$^{3}) =$\break 1 emu/cm$^{3}\to$  $ 4\pi \times  10^{-4}$ T \\
$\chi , \kappa $& 
Susceptibility& 
1 $\to  4\pi $ \\
$\chi_{\rho }$& 
Mass susceptibility& 
1 cm$^{3}$/g $\to  4\pi \times  10^{-3}$ m$^{3}$/kg \\
$\mu $& 
Permeability& 
1 $\to  4\pi \times  10^{-7}$ H/m   $= 4\pi \times  10^{-7}$ Wb/\break(A $\cdot$ m) \\
$\mu_{r}$& 
Relative permeability& 
$\mu \to \mu_{r}$ \\
$w, W$& 
Energy density& 
1 erg/cm$^{3} \to  10^{-1}$ J/m$^{3}$ \\
$N, D$& 
Demagnetizing factor& 
1 $\to  1/(4\pi )$ \\
\hline
\end{tabular*}
\label{tab1}
\end{table}

\subsection{Sentences and Paragraphs}

Write simply and clearly. Use clear and simple sentences, and arrange them in logical  order. A good rule of thumb is to try to minimize the use of colons, semicolons, quotation marks, and parentheses. Please strive for a smooth, linear writing style.

\begin{itemize}
\item Organize sentences into coherent paragraphs of reasonable length. A paragraph can be as short as one or two sentences but usually not longer than half of a page.

\item Organize paragraphs into sections, subsections, and subsubsections with common themes.

\item Give careful consideration to the section/subsection/subsubsection structure of your article.

\item A theorem or proposition is a single paragraph.

\item Indent every paragraph without exception. Use an indentation of 1 cm.

\end{itemize}

Carefully introduce terminology, and use your terminology consistently. Write with precision and clarity.

Use\enlargethispage{-12pt} the first part of your introduction to present your area of application to the readers. Do not assume that readers know anything about your application. Tell readers about the control  issues and challenges that arise and why these issues are relevant to your application. Use examples to illustrate these issues and\break challenges.

\subsection{Equations}

Display\enlargethispage{-12pt} equations should be centered and numbered consecutively, with equation numbers in parentheses and flush right. Refer to equations in text as (1), not eq. (1) or equation (1).

\pagebreak

Punctuate every equation as a smooth, integral part of the sentence, using commas and  periods as appropriate. That is, punctuate each equation as part of a sentence in a grammatically correct manner. A comma is used at the end of every equation in a list and use a comma at the  end of an equation that is followed by ``where.''

Do not precede equations with a colon. Do not use the word ``following'' (or the words  ``given by'') to introduce an equation. Do number all equations that you need to refer to. Number equations in the style (1), (2), (3). In \LaTeX{} this can easily be done using \verb|\eqref{label}|. Number an equation and refer to the equation by its number rather than writing ``the above equation.'' Do not use a single number to reference multiple equations. It is better to assign a separate number to each equation. Center every displayed equation. Try to avoid including words on the same line as a displayed equation. An exception is ``for all.'' Do not use the mathematical symbols $\forall$ to denote ``for all.'' Be absolutely sure that every symbol in every equation is precisely defined  with appropriate dimensions or\break units.

A good example is: It follows from Newton's second law
\begin{equation}
f = ma,\label{eq1}
\end{equation}
where $a$ denotes acceleration, that force is proportional to mass. Hence, 
\begin{equation}
a = f=m.\label{eq2}
\end{equation}

Note that \eqref{eq1} is an appositive and \eqref{eq2} provides the verb to the sentence.

\subsection{Tense}

It is usually possible to avoid the use of the future tense. Replace, ``This controller will solve many difficult problems'' with ``This controller can solve many problems.'' Some examples of good tense usage are

\begin{itemize}

\item These rules \textit{are} written for the benefit of \textit{IEEE CS}. 

\item The experimental results \textit{showed} the applicability of the method in this particular application. 

\item The results of [7] \textit{suggest} that saturation can degrade performance.

\item The results given in the next section \textit{show} that  the plant is nonlinear.

\end{itemize}

\subsection{Wordsmithing Suggestions}

Write factually, and err on the side of understatement. Avoid ``hype,'' that is, hyperbole. Use the words ``extremely, ``many,'' ``quite,'' and ``very'' sparingly. Do not use the word ``clearly.''

Avoid repetition. Do not repeat what you have already said. However, an exception to this rule is that figure captions must be written to summarize and highlight the main points in the  text. Consequently, repetition between the text and figure captions is encouraged.


Avoid rhetorical questions for which answers are not expected, such as ``What could be  more important than solving this problem?'' Avoid asking the reader questions to advance the presentation.

Avoid the word ``important.'' For example, do not say ``It is important for engineers to develop teraflop computers that cost under US\$100.'' However, it may be acceptable to  write, ``Inexpensive teraflop computers are important since they can facilitate real-time weather forecasting.'' However, it is much better to avoid judgments and write, ``Inexpensive teraflop computers can facilitate real-time weather forecasting.'' Let the reader decide whether something is important or not.

Do not use ``one'' as the subject of a sentence. OK: We expect to find that...

Not OK: One expects to find that...

Avoid starting sentences with ``There are'' or ``There is.'' Weak: ``There are many models that are ill conditioned.'' Stronger: ``Many models are ill conditioned.''

Avoid using the word ``generally'' and the phrase ``in general,'' which means ``often'' or ``usually'' but otherwise is imprecise.

Do not use ``as'' as a synonym for ``because'' or ``since.'' Never use the imprecise phrase ``a number of.''

The correct use of ``a,'' ``the,'' and ``this'' is challenging, especially for nonnative speakers of English. Think of ``a'' as meaning ``some,'' while ``the'' refers to a specific or unique object.  The adjective ``this'' refers to an object that has already been specified. Omit ``the'' when used twice in a row such as in ``The inverse and [the] transpose of the matrix A are given by (3) and  (4), respectively.'' Despite these simple rules, subtle cases can arise, although with some thought the correct usage usually becomes evident. In some cases, it is best to use neither ``the'' nor  ``a.'' Example: ``The algorithm is based on a colored noise model. A noise term is included in the state equation. The process noise $w$ has stationary statistics. Noise is known to degrade the  performance of estimation algorithms.''

\subsection{Acronyms and Abbreviations}

Acronyms are useful for streamlining the text. Define acronyms at the first opportunity, and then use the acronym consistently: ``A model reference adaptive controller (MRAC) was used for stabilization. This MRAC can be used to control uncertain systems.'' The following rules apply to the use of acronyms.

\begin{enumerate}

\item Define all acronyms except those that represent names of commercial products. Although MIMO, SISO, and PID are widely used, it is usually a good idea to define these acronyms.

\item To define an acronym, use the words first, followed by the acronym in parentheses. ``The nonlinear backstepping (NBS) controller stabilizes the system.'' Do not capitalize the words,  just the acronym.

\item Do not introduce an acronym that is not used subsequently. Avoid introducing an acronym that is subsequently used only one or two times.

\item Be conservative in introducing acronyms. The sentence ``The MV for the ODE was used in the MIMO PID FLC'' is painful to read.

\item Do not use acronyms in a figure caption unless an acronym appears in the figure itself, in which case, redefine the acronym in the caption even if it is already defined in the main text.

\item Do not use or define an acronym in a section or subsection heading.

\item It is acceptable to begin a sentence with an acronym.

\item If you develop a method or testbed, it may be extremely convenient to invent a name for the method or testbed, and refer to the method or testbed by its name. The name can then be shortened through the use of an acronym, which facilitates the discussion.

\end{enumerate}

Do not use ``etc.'' or ``and so forth.'' Do not use ``e.g.'' or ``i.e.'' Replace ``e.g.'' with ``for example,'' ``for instance,'' or ``such as,'' and replace ``i.e.'' with ``that is.'' Do not use ``vs,'' ``viz,'' ``cf,'' ``ca,'' or ``ibid.'' Do not use ``w.r.t.'' Rather, use ``with respect to.''

Do not use the mathematical symbols $\forall$ to denote ``for all,'' backwards $\exists$  to denote ``there  exists,'' or $\Rightarrow$  for ``implies.'' Use English words in mathematical statements.

Use ``U.S.'' as an adjective and USA for addresses.

\subsection{Punctuation}

Simple, short, and clear sentences can be highly effective. Semicolons (;) and dashes (--) are fine, but do not overuse them. Avoid lists that use bullets (\guillemotright). A few lists with or without bullets are acceptable from time to time, but try to write in text form. Your article is not a PowerPoint presentation.

Include the comma preceding ``and'' when referring to more than two items, such as $x$, $y$, and $z$. Please follow this rule consistently in your article. Likewise, write $x$, $y$, or $z$. A comma is needed to separate clauses in compound sentences, and this rule is universally followed. Omit the commas surrounding short appositives. For example, rewrite ``the state variable, $x$, is a vector'' as ``the state variable $x$ is a vector.''

\subsection{Italics, Quotation Marks, Apostrophes, and Bold}

Italics can be used for emphasis, but only very rarely. Use italics for all mathematical variables such as $x$ in \verb|$y = f(x)$|. Do not use italics for chemical compounds, atoms, and molecules such as NO and H$_2$O. Minimize the use of italics for emphasis and quotation marks for nonstandard language. Unlike the document you are reading, do not use bold font for emphasis.  Bold font can be used for math variables.

\subsection{Hyphens}

The rules for hyphens are reasonably logical but somewhat involved. This section provides examples of usage. When in doubt, do not use a hyphen. See ``Use of Hyphens'' for a longer list of words spelled without hyphens. Use hyphens for multiple modifiers such as ``computer-based
synthesis'' or ``Lyapunov-function analysis'' to show that the first word modifies the second word. The hyphen is also used in common phrases such as ``state-space model,'' ``nonminimum-phase zero,'' and ``first-order\break systems.''

``John is well known'' does not have a hyphen since ``is well known'' is the predicate. Likewise, a ``positive-definite matrix'' is hyphenated, whereas ``The matrix is positive definite'' is not hyphenated. The engineer ran a real-time simulation. The simulation runs in real time.  The positive-definite matrix satisfies the Riccati equation. The solution of the Riccati equation is positive definite. Note that a hyphen is not used in the\break predicate.

Use a hyphen in multi-axis, multi-input, and multi-output. The following words have  hyphens: all-weather, electro-optical, ground-based, in-flight, off-road, semi-empirical, tip-up. The prefix self requires a hyphen. Follow-up and close-up have hyphens. Use a hyphen in co-opt, co-owner, re-establish, and re-evaluate. 

Prefixes such as anti, bi, co, counter, de, ill, in, inter, intra, multi, non, off, on, out, over,  post, pre, proto, pseudo, quad, quasi, re, semi, sub, super, trans, tri, under, uni, and well might or might not warrant a hyphen. Likewise, suffixes such as based, by, down, fixed, free, in, ite,  less, off, out, up, and wise might or might not warrant a hyphen. When in doubt, do not use a hyphen.

Do not use a hyphen in coauthor, cochair, codirector, coeditor, cofounder, cooperate, coordinate, cosponsor, cosupervisor, coworker, and reinvent. Unlike the noun versions, the following verbs have no hyphen: back up, build up, close up, look up, ramp up, roll up, scale up, set up, shut down, speed up, spin up, start up, and\break trade off.

The following provides some further examples. The system has three degrees of freedom (DOFs). A six-degree-of-freedom (6DOF) robotic arm is used for the experiment. Note the  singular word ``degree'' in the latter phrase and the absence of a hyphen in 6DOF. The abbreviations 1D, 2D, and 3D have no hyphen. The testbed uses a 3-ft-long table. The table is 3-ft long. We use a 6-ft-by-6-ft test\break fixture.

\subsubsection{Capitalization}

When in doubt, use lower case letters. Do not capitalize names of technical items. For example, write ``linear-quadratic,'' but do not write ``Linear-Quadratic.'' Always capitalize  acronyms as in ``linear-quadratic (LQ).''

\begin{sidebar}{Use of Hyphens}
\sdbarinitial{N} ote the spelling of these words as single words with no hyphen: aeroelastic, aeroservoelastic, aimpoint, allpass, axisymmetric, backup, bandpass, bandlimited, bloodstream, breakpoint, buildup, colocated, coprime, countdown, counterclockwise, counterintuitive, counterproductive, crossover, cutoff, deadbeat, deadzone, drivetrain, electromechanical, feedback, feedforward, feedthrough, flyby, gearbox, geartrain, handheld, hardwired, ingoing, inline, interagent, interarrival, interrelated, liftoff, lightweight, longstanding, lookup, multidimensional, multidisciplinary, multilayer, multilevel, multimode, multimodel, multiobjective, multipath, multirate, multiscale, multistage, multistep, multivehicle, narrowband, nonadaptive, nonadditive, noncausal, noncolocated, nonconservative, noncontact, nonconvex, nondestructive, nondeterministic, nondissipative, nonempty, nonequilibrium, nonessential, nonferrous, nonholonomic, nonideal, noninvasive, nonlinear, nonlocal, nonminimum, nonnegative, nonoverlapping, nonrepeating, nonsquare, nonstandard, nonstationary, nontrivial, nonuniform, nonzero, offboard, offline, offset, offshoot, offsite, onboard, ongoing, online, onsite, outgoing, overcrowded, overparameterized, passband, piecewise, powertrain, preset, reinvent, rewritten, rolloff, rollover, rollup, roundoff, scaleup, setpoint, setup, shutdown, sideslip, speedup, spinup, startup, subdivision, suboptimal, subregion, subsection, substep, subsystem, swingby, swingup, teamwork, testbed, tradeoff, unidirectional, warmup, workpiece, worldwide.
\end{sidebar}

We write ``Editor George Smith'' and ``George Smith is the editor.'' Note the difference in capitalization due to the editor as a title or the name of the position.

Write ac and dc for AC and DC, and write cg for CG. Write Matlab and Simulink, not  MATLAB and SIMULINK. Capitalize Earth, Moon, Sun, and the names of all of the planets.

\subsection{Units}

Write units without italics and with a space after the number. Correct: ``3.57 mm.'' Wrong: ``3.57mm.'' IEEE CS uses ``s'' for second and ``h'' for hour. Also, use ``l'' (ell) for liter.

 Use ``bit'' for bit. Write ``US\$100'' or ``US\$100 million'' for money. Note the use of a hyphen in the units N-m, N-m-s, and kg-m2 and that this style is different from the standard SI style.

\subsection{Spelling}

The word ``affect'' is a verb. The word ``effect'' can be either a verb or a noun. Noise can affect the performance of the algorithm. The noise has an effect on the performance of the algorithm. A good leader can effect change in an organization. Verb, noun, verb.

Watch out for single and double ``ells.'' The system is modeled, and modeling is useful. The figure is labeled, and labeling is useful. The vehicle traveled and is now traveling. The system is controlled, the poles are canceled, and the instability is due to a cancellation. These spellings are not completely logical.

\textit{IEEE CS} uses ``parameterize'' and ``parameterization,'' not ``parametrize'' and ``parametrization.'' \textit{IEEE CS} uses queuing, not queueing. Replace spellings such as ``analyse, behaviour, centralise, centre, colour, diagonalise, emphasise, generalise, honour, optimise, practise, recognise, visualise'' with ``analyze, behavior,\vadjust{\vfill\pagebreak} center, centralize, color, diagonalize, emphasize, generalize, honor, optimize, practice, recognize, visualize.''



\begin{remark}
This is an example of a headline for paragraphs such as Lemma, Defintition, Proposition, Example, and Remark. 
\end{remark}

\begin{proof}
Here is an example of a proof subhead and paragraph.
\end{proof}

\section{CONCLUSION}

We hope that these files are useful to you in preparing your submission for \textit{IEEE CS}. We again remind you to carefully study the \textit{IEEE CS} Author's Guide. If you have any questions, do not hesitate to contact the editor-in-chief.


==> macros.tex <==
% 6 lines per inch allowed
\linespread{0.901}

% % Change section header font sizes
% \titleformat{\section}{\normalfont\fontsize{12}{15}\bfseries}{\thesection}{1em}{}
% \titleformat{\subsection}{\normalfont\fontsize{12}{15}\bfseries}{\thesubsection}{1em}{}
% \titleformat{\subsubsection}{\normalfont\fontsize{12}{15}\bfseries}{\thesubsubsection}{1em}{}

% \newtheorem{thm}{\textbf{Theorem}}
% \newtheorem{remark}{Remark}
% \newtheorem{lemma}{\textbf{Lemma}}
% \newtheorem{lem}{\textbf{Lemma}}
% \newtheorem{corol}{\textbf{Corollary}}
% \newtheorem{prop}{\textbf{Proposition}}
% \newtheorem{defn}{\textbf{Definition}}
% \newtheorem{example}{\textbf{Example}}
% \newtheorem{algo}{Algorithm}

\newcommand{\Red}[1]{\textcolor{red}{{#1}}}  % material to revise
\newcommand{\Blue}[1]{\textcolor{blue}{{#1}}}  % material to revise

% English 
\newcommand{\ie}{\textit{i.e. }}
\newcommand{\eg}{\textit{e.g. }}
\newcommand{\iid}{\textit{i.i.d. }}

% Probability
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}
\providecommand{\var}{\mathrm{Var}}

% Poisson
\newcommand{\pois}{\mathcal P}
\newcommand{\rate}{\gamma}

% Numbers 
\newcommand{\R}{\mathbb{R}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\ints}{\mathbb{Z}}
\newcommand{\compls}{\mathbb{C}}
\newcommand{\nats}{\mathbb{N}}

% SECTION 2 
\newcommand{\dt}{h}
\newcommand{\capa}{C}
\newcommand{\m}{Z}
\newcommand{\n}{n}
\newcommand{\nn}{\sigma}
\newcommand{\out}{M}
\newcommand{\cnoise}{v}

% SECTION 3
\newcommand{\de}{\delta}
\newcommand{\bx}{\bar x}
\newcommand{\bu}{\bar u}
\newcommand{\diff}{\frac{d}{dt}}
\newcommand{\bits}{\mathcal R}
\newcommand{\lbits}{\mathbb M}

% \DeclareMathSymbol\bbDelta  \mathord{bbold}{"01}
% \newcommand{\linf}{\ell_\infty\rightarrow\ell_\infty}

% \renewcommand{\dateseparator}{.}
\long\def\/*#1*/{}
\newcommand{\myf}{\hspace{-0.1em}f}
\newcommand{\Phihat}{\hat{\Phi}}
\newcommand\inner[2]{\langle #1, #2 \rangle}
\newcommand\optx[3]{\begin{alignat}{2}& \underset{#1}
{\text{minimize}}
& #2 \\\nonumber
& \text{subject to \ }
& #3\nonumber\end{alignat}}
\newcommand\optxnc[2]{\begin{alignat}{2}& \underset{#1}
{\text{minimize}}
& \ \ #2 \\
\end{alignat}}

\newtheoremstyle{named}{}{}{}{}{\bfseries}{.}{.5em}{\thmnote{#3} Principle}
\theoremstyle{named}
\newtheorem*{namedprinciple}{Principle}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}

% signals
\def\u{\mathbf{u}}
\def\w{\mathbf{w}}
\def\x{\mathbf{x}}
\def\K{\mathbf{K}}

\def\R{\mathbf{R}}
\def\M{\mathbf{M}}

\renewcommand{\vec}[1]{\boldsymbol{#1}}

==> packages.tex <==
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage[bbgreekl]{mathbbol}
\usepackage[yyyymmdd]{datetime}
\usepackage[margin=1in]{geometry}
\usepackage[T1]{fontenc}
\usepackage[skip=2pt,font=footnotesize]{caption}
\usepackage{titlesec}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage[numbers,sort&compress]{natbib}
\usepackage{graphics}
\usepackage{hyperref}
\usepackage{multirow}
\usepackage{tikz}
\usepackage{bibentry}
\usepackage{nccmath}
\usepackage{wrapfig}

\usepackage{booktabs,amsfonts,algorithmic,algorithm2e,mathtools,framed,pbox,color,mathrsfs}

==> tex-files/bode.tex <==
\setcounter{sequation}{0}
\renewcommand{\thesequation}{S\arabic{sequation}}
\setcounter{stable}{0}
\renewcommand{\thestable}{S\arabic{stable}}
\setcounter{sfigure}{0}
\renewcommand{\thesfigure}{S\arabic{sfigure}}
\section{Bode'S Integral: A Measure of Robustness} \label{sec:robustness}


   \sdbarfig{\label{fig:InvertedPendulum_block}
    \includegraphics[clip =true,  trim=3.3cm 4.5cm 3.3cm 6.5cm, width = .7\linewidth]{figures/IPblockdiagram.pdf}}{\footnotesize A linear feedback system.}   


The following is adapted from~\cite{leong2016understanding}. Robust control theory studies the effects of uncertainties in a system, quantifying the system's fundamental limitations or \emph{laws}. More precisely, robust control theory focuses on understanding the amplification of noise, termed robustness, in a closed-loop system and the impacts of unstable poles, unstable zeros, and delay on robustness using the $H_\infty$ norm and the Bode's integral \cite{doyle2013feedback}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Sensitivity Functions}

Sensitivity functions are quantities of interest in robust control theory because they are transfer functions from noise to the closed-loop system output. Effectively, they quantify the amplification of noise in a closed-loop system. To obtain the sensitivity functions, the closed-loop output $\hat{z}$ (see Fig. \ref{fig:InvertedPendulum_block}) can be written as
% \begin{sequation}
% 	\hat{z} = \frac{((l-l_0)s^2 - g) \;\hat{r} - C(s)((l-l_0)s^2 - g)\;\hat{n} }{D(s)+((l-l_0)s^2 - g)C(s)}. \label{eq:clz}
% \end{sequation}
\begin{sequation}
	\hat{z} = \frac{P(s)}{1+P(s)C(s)e^{-\tau s}}\hat{r} - \frac{P(s)C(s)e^{-\tau s} }{1+P(s)C(s)e^{-\tau s}} \hat{n}, \label{eq:clz}
\end{sequation}
% \begin{sequation}
% 	\hat{z} = \frac{((l-l_0)s^2 - g)}{D(s)+((l-l_0)s^2 - g)C(s)} \hat{r} - \frac{C(s)((l-l_0)s^2 - g) }{D(s)+((l-l_0)s^2 - g)C(s)}\hat{n}. \label{eq:clz}
% \end{sequation}
where $s$ is the complex Laplace variable, and $\hat x$ denotes the Laplace transform of $x$.

Define the sensitivity function, $S(s)$, and the complimentary sensitivity function, $T(s)$, \cite{doyle2013feedback} as
\begin{align}
S(s) = \frac{1}{1+P(s) C(s) e^{-\tau s}}, \quad
% & =  \frac{D(s)}{D(s)+((l-l_0)s^2 - g)C(s)}
% \end{align}
% \begin{align}
T(s) = \frac{P(s) C(s)e^{-\tau s}}{1+P(s) C(s)e^{-\tau s}}. \label{eqn:T} 
% & =  \frac{((l-l_0)s^2 - g)C(s) e^{-\tau s}}{D(s)+((l-l_0)s^2 - g)C(s)}. \label{eqn:T}
\end{align} 
Then, \eqref{eq:clz} can be rewritten as
\begin{equation*}
	\hat{z} =  P(s)S(s)\hat{r} - T(s) \hat{n}\label{eq:clperformance}.
\end{equation*} 
If $T(s)$ and $S(s)$ is small, for any given noises $r$ and $n$, the deviation $z$ will also be small. Note that given an unstable pole $p$ and an unstable zero $q$ of the plant $P$,
\begin{sequation}
	S(q) = 1 \qquad T(p) = 1, \label{eq:st-one}
\end{sequation}
an important fact that is used later.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{$H_\infty$ Norm}\label{sec:hinf norm}
 % Note that given a RHP pole $p$ and a RHP zero $z$, then
% \begin{sequation}
% 	S(z) = 1 \qquad T(p) = 1. \label{eq:st-one}
% \end{sequation}
The deviation $z$ of the system from the equilibrium point is desired to be small for any given noises $r$ and $n$. Hence, we define the performance measure of the system as a norm of the closed-loop transfer functions $T(s)$ and $S(s)$ from noise sources to $z$. The infinity ($H_\infty$) norm of a transfer function is defined as
\begin{equation*}
	\norm{G}_{\infty} = \sup_\omega |G(j\omega)| = \sup_{Re ~ s >0} |G(s)|
\end{equation*}
where the last equality is given by the Maximum Modulus Theorem \cite{doyle2013feedback}.  By this definition, a system is robust when the infinity norm of $T(s)$ and $S(s)$ are small (i.e. when the magnitude of the transfer function at all frequencies is small). 

In sensorimotor applications, which we discuss in greater detail in later sections, the impacts of the measurement noise and the actuation noise (e.g., neural signal noise during muscle activation) on system robustness are similar, but the feedback delay will only amplify the measurement noise. Hence, we assume that the limiting factor is the sensing noise and the analysis henceforth will focus on $T(s)$. Nonetheless, similar analysis can be applied to study the effect of actuation noise. The infinity norm of $T(s)$ can be shown (see~\cite{doyle2013feedback,leong2016understanding}) to satisfy
\begin{gather}
\ln \norm{T(s)}_{\infty} \geq F \triangleq  % MathType!MTEF!2!1!+-
\tau p + \ln \left| {\frac{{p + q}}{{p - q}}} \right|,
 \label{eqn:hinfT} 
\end{gather}
where $T(s)$ is the transfer function from measurement noise $n$ to output $z$ given in \eqref{eqn:T}, $F$ is the system fragility, $p$ is an unstable pole, $q$ is an unstable zero, and $\tau$ is the total delay in the control system from measurement to actuation.

The $H_\infty$ norm quantifies the worst case noise amplification, and the lower bound $F$ provides the smallest possible worst case noise amplification, the fundamental limit, or \emph{law}, of this system independent of the controller. In engineering, given this information, system engineers decide on whether this fundamental limit is acceptable. If not, the system needs to be redesigned. In sensorimotor control tasks, the fundamental limit defines a human's best performance in the task using the noisy nervous system regardless of the decision making process of the brain.

\hfill\emph{(continued on next page)}
 \end{sidebar}

\begin{sidebar}{\continuesidebar}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bode's Integral: A Law for Feedback Control Systems}

Similar to the $H_\infty$ norm, the Bode's integral places a hard lower bound on the net achievable robustness of a control system in the presence of measurement noise. A small integral implies a less fragile (i.e. more robust) system is possible, and sensor noise does not necessarily prevent stabilizing the system. %In other words, given a particular stick balancing task, the smallest possible amplification effect of the visual measurement noise is given by the fragility $F$. 
% This section introduces the Bode's integral.
\begin{no-theorem} \label{lem:bodeintegral}
The Bode's integral is given by
\begin{sequation}
\ln |G_{mp}(s_0)| = \frac{1}{\pi}\int^\infty_{-\infty} \ln |G(j\omega)| \frac{\sigma_0}{\sigma_0^2+(\omega-\omega_0)^2} d\omega \label{eq:bode0}
\end{sequation}
where $s_0 = \sigma_0+\omega_0 j$ with $\sigma_0 > 0$, $G(s)$ is any transfer function, and $G_{mp}(s)$ is a minimum phase transfer function of $G(s)$. 
\end{no-theorem}
In the case of a plant with an unstable pole $p$, unstable pole $q$, and delay $\tau$, the Bode's integral of $T(s)$ is bounded as follows.
\begin{no-theorem} \label{thm:bodeintegral}
The Bode's integral of $T(s)$ is bounded by
\begin{gather}
	\frac{1}{\pi}\int^\infty_{-\infty} \ln |T(j\omega)|~ \frac{p}{p^2+\omega^2} ~d\omega \ge F
	% p = \sqrt{\frac{(M+m)g}{M l}} \qquad \quad q  = \sqrt{\frac{g}{l-l_0}} \nonumber
% \frac{1}{\pi}\int^\infty_{-\infty} \ln |T(j\omega)| \frac{p}{p^2+\omega^2} d\omega \geq \tau p + % MathType!MTEF!2!1!+-
% \left\{ {\begin{array}{*{20}{c}}
% 0&{{l_0} \ge l}\\
% {\ln \left| {\frac{{z + p}}{{z - p}}} \right|}&{{l_0} < l}
% \end{array}} \right.
\label{eq:bode}
\end{gather}
where $T(s)$ is the transfer function from measurement noise $n$ to output $z$ given in \eqref{eqn:T}, $F$ is the system fragility, and $p$ is the unstable pole. $F$ and $p$ are defined as in \eqref{eqn:hinfT}.
\end{no-theorem} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The Waterbed Effect}

The Bode's integral is a conserved quantity that exhibits the waterbed effect. If $T(s)$ is small for a certain frequency range, then at some other frequency range, $T(s)$ will necessary be large, similar to a waterbed whereby one side will rise when you push at the other side. More precisely,

\begin{no-theorem}[Waterbed Effect]\label{thm:waterbed}
Suppose that a plant $P(s)$ has an unstable pole $p$. Then, there exist positive constant $c_1$ and $c_2$, depending only on $\omega_1$, $\omega_2$, and $p$, such that
\begin{sequation} 
	c_1 \ln M_1 + c_2 \ln M_2 \ge \ln \mid T_{ap}(p) \mid^{-1} \ge 0
\end{sequation}
where $[\omega_1,\omega_2]$ defines some frequency range, $T_{ap}(s)$ is the all-pass complimentary sensitivity function for the plant $P(s)$, $M_1 = \max_{\omega_1 \le \omega \le \omega_2} |T(j \omega)|$ and $M_2 = \norm{T(s)}_\infty$.
\end{no-theorem}

% \begin{proof}
% %Proof is available at \cite{doyle_dft}.
% Let $p = \sigma_0+j \omega_0$ and recall that $T_{mp}(p)=T_{ap}(p)^{-1}$. Then, from Lemma \ref{lem:bodeintegral},
% \begin{align*}
% 	\ln |T_{ap}(p)^{-1}|& = \frac{1}{\pi}\int^\infty_{-\infty} \ln |T(j\omega)| \frac{\sigma_0}{\sigma_0^2+(\omega-\omega_0)^2} d\omega \nonumber \\
% 	& \le c_1 \ln M_1 + c_2 \ln M_2. 
% 	%&= \ln\left( \left|\frac{z+p}{z-p}\right| e^{\tau p}\right) \nonumber.
% \end{align*}
% where $c_1$ is the integral of $\frac{1}{\pi}\frac{\sigma_0}{\sigma_0^2+(\omega-\omega_0)^2}$ over the domain $[-\omega_2,-\omega_1] \cup [\omega_1,\omega_2]$ and $c_2$ is the same integral over the complimentary domain.
% By Maximum Modulus Theorem, $|T_{ap}(p)^{-1}| \le 1$. Thus, $\ln |T_{ap}(p)^{-1}| \ge 0$.
% \end{proof}

Next, we use the \nameref{thm:waterbed} to derive another law for the control system illustrated in Fig.~\ref{fig:InvertedPendulum_block}.
\begin{no-theorem}\label{thm:waterbedip}
	The complimentary sensitivity function $T(s)$ satisfies
\begin{sequation} 
	c_1 \ln M_1 + c_2 \ln M_2 \ge F 
\end{sequation}	
where $F$ is the system fragility defined as in \eqref{eqn:hinfT}, $M_1 = \max_{\omega_1 \le \omega \le \omega_2} |T(j \omega)|$, $[\omega_1,\omega_2]$ defines some frequency range, $M_2 = \norm{T(s)}_\infty$, and $c_1$ and $c_2$ are constants that depend only on $w_1$, $w_2$, and $p$.
\end{no-theorem}

% \begin{proof}
% 	Recall that $T_{ap}(p)^{-1} =  \frac{p+q}{p-q}e^{\tau p}$ when there is a RHP zero $q$, and $T_{ap}(p)^{-1} = e^{\tau p}$ when there is no RHP zero. The rest follows from simple algebraic manipulations.
% \end{proof}

Thus, if amplification $T(s)$ is small for some frequency range, i.e., if $M_1$ is small, then, by the \nameref{thm:waterbed}, $M_2$ has to be large, implying that $T(s)$ is large at some other frequency. Therefore, if $F$ is large, the system cannot have small $T(s)$ at all frequency. Furthermore, as the bound $F$ increases, the peak of $|T(s)|$ is likely to increase at some frequency. 


==> tex-files/gnc-vignette.tex <==
\sdbarinitial{L}ayered architectures have been central to Guidance, Navigation, and Control (GNC) since its inception as a field of study.  Remarkably, despite dramatic advances in sensing and computing capabilities, the overall structure depicted in \label{fig:apollo}, taken from \cite{apollo}, remains mostly unchanged.

\sdbarfig{\includegraphics[width=38.0pc]{figures/gnc-apollo.pdf}}{Figure taken from~\cite{apollo}, showing the proposed GNC architecture. 
 In contrast to the GNC literature, we explicitly delineate mission planning (decision making) from tajectory planning.  Nevertheless, the vertical decomposition across time-scales and complexity is present. \label{fig:apollo}}




==> tex-files/history.tex <==
history of architectures goes here

==> tex-files/intro.tex <==
% {\bf This is a rough cut mostly for internal consumption but is close to what I hope to start with...  there sill be some brief paragraphs at the end as noted, but this is most of it.  Wanted to clarify from standard modern usage centrality of layers and the distinction between abstract and virtual.}

% The claim that there are universals in layered architectures despite the obvious diversity in systems that deploy them seems paradoxical but is in fact the essence of why we have architectures, to enable functional diversity that can’t be directly implemented in simple available components.  We aim to explain this using two distinct starting points that we hope will converge.  One is the shared universals in the extant architectures that dominate our world, all evolved by natural selection. Unfortunately, a shared universal most in need of theory is intelligent design of upgrades that address the ubiquity of fragility and unsustainability in our most important architectures.  The other starting points are the existing theories in control, communications, computing, and physics that are initially incompatible but hopefully complementary, particularly when viewed from an architectural perspective. The ultimate goal is to have a unified theory.

The familiar evolution of control theory can be viewed as an elaboration of layers, though this is not standard. In classical control, the layering of control/plant (C/P) was an early abstraction of a common feedback design problem.  This can be expanded to explicitly focus on models of the environment (E) where most typical uncertainty arises, resulting in a C/P/E layered abstraction.  Then laws like \nameref{sidebar:bode}~\cite{doyle2013feedback} and the internal model principle~\cite{francis1976internal} were added.  In aerospace in particular, this was further elaborated by stacking navigation (N) and guidance (G) layers on top of control for N/G/C/P/E layers, see Fig.~\ref{fig:layer-apollo} and \citet{kendoul2012survey}. More generally the layering of decision/trajectory/feedback (D/T/F) give a more universal D/T/F/P/E layering that has ubiquitous applications in technology and science, see Fig.~\ref{fig:three_layers}.

\begin{sidebar}{Bode's Integral: A Law for Feedback Control Systems}
\section[Bode's Integral Formula]{}\phantomsection
\label{sidebar:bode}
\input{tex-files/bode}
\end{sidebar}

\setcounter{equation}{0}

While we define and explain key concepts in control architectures, such as layers, in detail in the next section, we instead here provide a general and historical perspective on both the development and usage of these shared universals across different fields. 
%
The most important general concept to clarify is \emph{layers}. Layers exist in control theory, but are most explicitly the focus of the theory of computing. Computing is important in control because we need methods whose algorithms scale gracefully with system size and complexity, and the high layers in all of our control systems run on digital computers.  Fortunately, computing has arguably had the richest treatment of layering and this will be central to any general theory of architecture.

We can draw some important insights even from a superficial, highly simplified, modern, and ahistorical view of the subject. 
%that will hopefully be familiar and have errors easily fixed by those who are experts.  
We can think of layering theory as starting with Turing’s split of computing into data/HW, where HW denotes some fixed hardware that implements some algorithm, and data is the external input to and output from the algorithm.  The (nonstandard) notation data/HW will be used throughout to describe layers. Here it succinctly emphasizes the layering, and that diverse algorithms in HW can act on a vastly greater diversity of data, but all with this shared universal architecture. 

Turing then elaborated on this by brilliantly splitting data into (data/SW)/HW where HW now is a universal Turing machine (UTM)~\cite{turing1936computable} that can emulate all HW and the algorithms are now in software (SW) which is just a special kind of data. This means that in principle a single HW UTM can run SW as diverse as the HW in the original data/HW architecture by treating the algorithm as data.  Turing then could prove a hard law on computation, in that some problems were decidable (could be computed on a Turing machine) and some were undecidable (could not finish in finite time)~\cite{turing1954solvable}.  The field of computational complexity~\cite{arora2009computational} has become one of the richest in mathematics and engineering, and is essential to a theory of layered (control) architectures, since constraints on offline and online computation are as serious as any from traditional control theory (e.g. Bode).  

\newcommand{\HALT}{\texttt{HALT}\space}
The starting point for computational constraints and one of the most significant results of the 20th century is Turing's proof that the Halting Problem was undecidable~\cite{turing1936computable}.  Specifically, Turing proved that in the data/SW/HW architecture, abstracted as a UTM, one could propose a \HALT algorithm that could take any other algorithm and compute whether it ever halted. Turing proved that no such \HALT algorithm existed, making Halting and a surprisingly large set of naively stated problems undecidable with UTMs.   This has spawned one of the deepest theoretical and practically relevant research communities on computational complexity in layered computing architectures.  The Internet in particular elaborated on this architecture with additional layers and networking, see~\cite{chiang2007layering} and references within, as well as Fig.~\ref{fig:layer-tcpip}.

The SW in data/SW/HW can be viewed as creating a virtual version of the HW as seen from the data.  We use \emph{virtualization} to describe the consequences from the perspective of data in the real world implementation of this architecture, and reserve \emph{abstraction} for the language and mathematics used to describe, model, analyze, and design architectures and the systems that use them. 
%
An example of the distinction between abstract and virtual is memory.  Turing machines have a severe abstraction of memory by assuming it is infinite and focusing on the time complexity of algorithms. Even today, this is a reasonable starting abstraction as memory is relatively cheap, completely reusable, and a powerful resource (e.g., PSPACE=NPSPACE), particularly in contrast with time. In practice, memory is highly virtualized with layers of SW/fast-small/slow-large memories with SW algorithms creating a virtual memory that appears fast and large even with no component part that is.  
%
This virtualization is a simple example of laws and a Diversity enabled Sweet Spot (DeSS).  There is great diversity in the memory hardware but there is a \emph{law} that for a fixed budget only fast-small or slow-large memories are available and not large-fast.  This diversity ``enables'' virtual memories that have a sweet spot in speed and size but needs complex architecture and software to realize this, which is the essence of layering and virtualization.  

%% we're skipping this
%Hence DeSS and not merely \nik{DSS} is what drives the need for architecture. \nik{What's a DSS?}

% \nik{DSS is bad here, sorry.  Here's the point and need to make it more clearly but not waste a lot of space.}   DSS= Diversity Sweet Spot.  This is what I first called this.  But Marie said diversity doesn't create sweet spots, architecture does... but diversity is also essential for SS, thus DeSS.  We could just skip this point, but would like to say that "enabled" is used because the diversity is necessary but sufficient for SS, and you need architecture, hence DeSS.  Probably overly pedantic to even explain this as the readers should think this is obvious.  I'm ok with leaving this out or putting in something short and clear that I've been unable to figure out...

The usage of \emph{law} to include both undecidability and limits on physics as well as manufacturing is arguably overly broad and sloppy, and we might use adjectives as in mathematical law and technological law and/or use \emph{constraint} in place of \emph{law}. All involve tradeoffs, but unlike layers and virtualization, there is no commonly clear distinction between constraints, tradeoffs, and laws.%, and this is a topic that could use refinement.

Communications (i.e., information) theory beginning with Shannon~\cite{shannon1948mathematical} also has a layered interpretation that is natural but nonstandard.  Naively, an informative message would be meaningful, timely, and surprising.  Shannon brilliantly recognized that a theory could be built from just surprise, and this could be a key enabling protocol in a meaning/timely/surprise architecture.  For surprise (i.e., information), Shannon proposed source/channel layers, proved laws and hard limits on achievable communication, and optimal codes that realized these limits.  As in computing, this provides a key enabling protocol, here for communication, as in the original phone system that allowed people in diverse and remote locations to converse in real time. 

% \nik{what do you mean by platform here? seems like you're using this in the same way you use protocol/virtualization?}  Agree this is confusing, but could be important. We tend to reserve platform for a special component within a layer that effectively creates a new layer and a new virtualization.  Search is "just" an app in the app/OS/HW layering but has become effectively a new layer which we call a platform.  Arguably email, VPN, maybe Overleaf, VoIP, Amazon, Facebook, etc are platforms whereas most apps on my phone and PC are not... Server farms with GPUs etc could also be a platform.  A new OS would be the ultimate platform but would be really hard to do now, an example of the constraints on the "waist"  .... so platforms create new waists... so platforms are great examples of evolvability but might be subtlety we can skip.. but they are everywhere and most modern billionaires are so because they introduced or hijacked a platform.  I'm ok dropping this or trying to make it work.  As is, it is just confusing to readers who don't already know what I mean. The most important theory for platform started with Turing going from data/HW to data/SW/HW... and the next leap was data/apps/OS/HW... but there are lots of less significant even bad platforms, like twitter.

The abstractions that Turing and Shannon made were to focus on time and space, respectively, and integration of these abstractions and the laws that they define with control theoretic abstractions and laws (e.g., Bode) has proved challenging. Yet it is essential to a theory of architecture as timely, accurate and efficient computing and communication is essential to robust layered control of large systems.  Fortunately, exciting process has been made in the past decade, both in deriving integrated laws (see~\cite{martins2007fundamental, martins2008feedback,Nakahira2021}) and in explicitly accounting for communication channels and delay in \nameref{sidebar:dist-and-NCS}.

An important complement to layers and levels is {\it stages} which involve the flow of energy, materials, or data in networks and supply chains.  This term is standard in supply chain management and operations research and there is relatively little confusion about it. The important point here is that stages often have bowties that facilitate virtualization, robustness, and evolvability as discussed below.

With this multi-disciplinary and historical perspective in hand, the next section provides more concrete and familiar examples of the concepts alluded to so far.

\begin{sidebar}{Distributed and Networked Control Systems}
\section[Distributed and Networked Control Systems]{}\phantomsection
\label{sidebar:dist-and-NCS}
\subsection{Distributed Control}
     Although not the main focus of this paper, another key aspect of control architectures is their distributed nature.  Indeed, when applied to large-scale cyber-physical systems, distributed control solutions are needed. In distributed control, control systems are composed of several sub-controllers, each equipped with their own sensing, actuation, and compute---these sub-controllers then exchange local sensor measurements and control actions via a communication network.  This information exchange between sub-controllers is constrained by the underlying properties of the communication network, ultimately manifesting as information asymmetry among sub-controllers.  This information asymmetry is what makes distributed optimal controller synthesis challenging \cite{1972_Ho_info,2012_Mahajan_Info_survey,2006_Rotkowitz_QI_TAC,2002_Bamieh_spatially_invariant,2005_Bamieh_spatially_invariant,2013_Nayyar_common_info}---indeed, early negative results gave reason to suspect that the resulting distributed optimal control problems were intractable \cite{1968_Witsenhausen_counterexample,1984_Tsitsiklis_NP_hard}. These negative results, although not viewed as such at the time, represented hard limits, or laws, on efficient synthesis of distributed controllers.  As would be discovered in subsequent work, these laws were imposed by the cyber and physical levels of the system.
     
     Indeed, in the early 2000s, a body of work \cite{2002_Bamieh_spatially_invariant, 2004_QI, 2004_Dullerud, 2005_Bamieh_spatially_invariant, 2006_Rotkowitz_QI_TAC, 2012_Mahajan_Info_survey, 2013_Nayyar_common_info} culminating with the introduction of quadratic invariance (QI) in the seminal paper \cite{2006_Rotkowitz_QI_TAC}, showed that for a large class of practically relevant systems, the resulting distributed optimal control problem is convex.  A common theme among these conditions is the notion of having \emph{compatible structure} between the system dynamics and distributed control system communication network: loosely speaking, distributed control architectures, defined here in terms of actuation, sensing, and communication, that are at least as dense as the underlying physical system lead to tractable control problems. QI led to an explosion of synthesis results in this area \cite{2012_Lessard_two_player,2010_Shah_H2_poset,2013_Lamperski_H2,2013_Lessard_structure,2013_Scherer_Hinf,2014_Lessard_Hinf,2014_Matni_Hinf,2014_Tanaka_Triangular,2014_Lamperski_state, fattahi2019transformation}.  These results showed that the robust and optimal control methods that were proven so powerful for centralized systems could be used in distributed settings.  However, they also made clear that the synthesis and implementation of QI distributed optimal controllers did not scale gracefully with the size of the underlying system---indeed, the complexity of computing a QI distributed optimal controller is at least as expensive to compute as its centralized counterpart, and can be more difficult to implement. These problems are further compounded in the MPC setting where sub-controllers must solve optimization problems in near real-time. 

Motivated by this lack of scalability, the system level synthesis (SLS) approach to distributed control~\cite{wang2019system,wang2018separable,anderson2019} was developed. By considering an alternative closed-loop map, SLS provides an affine system parameterization which is more suited to distributed control. Indeed, SLS characterizes the largest known class of distributed control problems that admit a convex programming solution. Crucially, under additional assumptions, SLS provides a distributed control synthesis algorithm that scales independently of the state dimension of the network to be controlled. Following SLS, there has been a renewed interest in identifying alternative parameterizations of distributed stabilizing controllers, each applicable under different assumptions~\cite{furieri2019input,sabuau2021network}. 

\hfill\emph{(continued on next page)}
\end{sidebar}
\begin{sidebar}{\continuesidebar}

\subsection{Networked Control Systems}
An underlying assumption in all of the above is that information,
albeit delayed, can be transmitted \emph{perfectly} across a communication
network with a \emph{fixed} delay, i.e., that through an appropriate communication layer, the underlying communication network is virtualized with only fixed delays exposed to the control layer. 
%
A realistic communication network,
however, is subject to data rate limits, quantization, noise and packet
drops---all of these issues result in possibly varying
delays (due to variable decoding times) and imperfect transmission
(due to data rate limits/quantization).  The assumption that these delays are fixed necessarily
introduces a significant level of conservatism in the control design procedure.
In particular, to ensure that the delays under which controllers 
exchange information do not vary, worst case delay times must be used
for control design, sacrificing performance and robustness in the process.

These issues have been addressed by the networked control
systems (NCS) community, leading to a plethora of results for channel-in-the
loop type problems.  For example,
\cite{EM11,HOV02,NE03,TM04,WB99} identify minimum bit-rate conditions
sufficient to stabilize a system in the almost sure sense through
feedback control over a data-rate constrained channel. In \cite{Sahai01},
anytime capacity was identified as the correct metric for additionally
ensuring moment stability. Performance and robustness results also
exist, such as elegant extensions of the well known \nameref{sidebar:bode} to quantify the effect of channels in the loop \cite{martins2007fundamental,martins2008feedback}
on performance limits.
%
A complementary line of work~\cite{LA04,NH05,TM04,YQP04,ZBP01}
addresses the design of stabilizing feedback controllers subject to
either varying communication delay or packet drop outs. \citet{GSHM08} address optimal
LQG control of a single plant over a packet dropping channel. We refer
the interested reader to the excellent survey paper \cite{Hesp} for
a more complete overview of the state of NCS.

While less explored, there is also some work that seeks to combine NCS theory with distributed (optimal) control.  For example, in \cite{matni2013communication, Matni_Comms_TCNS}, methods are proposed which co-design a distributed optimal controller and the communication, actuation, and sensing architectures needed to implement it, under the assumption of perfect but delayed communication.  In complementary work~\cite{matni2013optimal,matni2014optimal} an explicit solution to a two player distributed LQR problem in which
communication between controllers occurs across a communication link with varying delay is presented.

\subsection{Layered architectures}
Distributed and networked control systems remain an active area of research, both of which stand to substantially benefit from adopting a vertical layered perspective that incorporates decision making and planning to complement the current horizontal decomposition of decision and control within the feedback control layer and vertical layering between communication and control.
\end{sidebar}



%\nik{Actually much is done already in controls. The earliest and most immediate impact has been to include comms/comp limits in Bode IF.  Lots of cites on this, the most trivial is the extension to Bode just to include delays (don't know who first did this but it was the 80s.  Freudenber?)  And the biking game distills the essence. Then SLS includes comms/comp limits explicitly.  This is all really important, perhaps one of the most important themes in the subject, but need to capture it better.  Suggestions?  Where should we put this? }

%% New philosophy: if you don't give me coherent material to integrate into the introduction, I'm cutting it.  We can add more when we revise.
% Much progress has been made in recent years in methods to design robust and scalable control systems constrained by limits on computing and communications, particularly sparsity and delay.  \nik{this is just kind of dangling.. and needs elaboration from Bode-Shannon to SLS... the glass is half full and I'm just saying it is half empty... but the half full is huge, and currently SLS is the new "platform"... this needs to be much clearer...}

% {\bf Need to add lots of citations}

% So need to say something about how layers and levels are orthogonal but even more confusing than virtual and abstract.  None of these terms are really standard but where they are used together and systematically, there is a universal meaning.  But mostly they are all mixed up in a soup of confusion, and at the risk of being pedantic, dogmatic, and Procrustean, we'd like to fix this.  




==> tex-files/learning-sidebar.tex <==

\begin{sidebar}{Learning in Layered Control Architectures}
\section[Learning in Layered Control Architectures]{}\phantomsection
\label{sidebar:learning}
A discussion on the role of learning in control architectures is conspicuously missing from \nameref{sec:layering}.  This absence is deliberate, as it is impossible to do justice to both the existing results and open questions in this area without significantly expanding the scope of this paper.  To that end, we instead provide an extremely brief and incomplete summary of learning in layered control architectures, with a focus on results from the robotics community that use learning to integrate rich perceptual sensors (e.g., cameras) and rich tasks (e.g., as specified through the objective of a (PO)MPD) into layered architectures for continuous control. 

\paragraph{The Learning-Enabled-Control Architecture Design Space} 
Two philosophically opposed approaches to designing suitable perception/action pipelines dominate both practice and theory: (i) layered, and (ii) end-to-end \cite{bojarski2016end,pomerleau1989alvinn,levine2016end}. The familiar layered approach, which is aligned with the overall theme of this paper and is rooted in engineering best-practices, designs different layers (perception, prediction, localization, planning, control) independently, and interconnects them via pre-specified (rigid) protocols. While the benefits of such approaches are well known to the controls community, and are also well suited to large organizational structures, this approach limits interaction between layers to often ad-hoc specifications shared between teams, thus limiting end-to-end optimization \cite{zeng2019end}.  
The end-to-end approach, classically favored by the deep reinforcement learning community, in contrast seeks to learn an optimized map directly from pixels (or other high-dimensional sensory inputs) to actions.  While such approaches have the advantage of optimizing the full perception/action pipeline for a specific application, and have led to impressive demonstrations, the resulting systems are opaque, difficult to troubleshoot, and lack safety guarantees.  Further, they often preclude prior knowledge from being incorporated into learning/design, leading to increased sample complexity and brittle algorithms.

These two approaches can be viewed as extreme points of a broader architectural design space, with the layered approach optimizing for interpretability, modularity, and (arguably) safety/robustness, and the end-to-end approach optimizing for performance and simplicity (of implementation).  A coherent theory of architecture will allow for a principled exploration of the entire design-space.  Indeed, existing work in the robotics and machine learning community, in particular in the context of safety-critical applications such as autonomous vehicles (AV), have recognized the need for diversity enabled architectures.  

For example, the robotics community has recently begun to explore similar questions to those raised in this manuscript, seeking to shift to an intermediate design philosophy. In the AV community, \cite{zeng2019end,liang2020pnpnet,luo2018fast,sauer2018conditional,williams2018information} propose end-to-end learnable motion planners, that take as input raw perceptual data (e.g, pixels or LIDAR), and produce both interpretable intermediate representations in the form of 3D detections and a space-time cost volume that is optimized via sampling by the planner.  In the context of agile perception based flight, recent work \cite{kaufmann2018deep} combines a CNN for perceptual sensing, which maps raw images to waypoints and desired speeds, which are then used by a planning module to generate short trajectory segments and corresponding motor commands to reach the desired goal. 

These preliminary results highlight two important points. First, that two independent sub-communities within robotics have converged to and discovered similar design pipelines highlights both the importance of architectural choices in learning-enabled-control systems, and the \emph{need for a unified underlying theoretical and algorithmic framework} for making these design choices.  Second, the \emph{choice of representations shared between perception and action components, i.e., the protocol, is an important design decision}: indeed, as described in \cite{kaufmann2018deep}, sharing discrete navigation commands as in \cite{kim2015deep,loquercio2018dronet} improves robustness at the expense of performance, and conversely, representations at the level of direct control \cite{kahn2017plato} can lead to highly agile control at the expense of high sample complexity and system fragility.  These are concrete examples of designed interfaces/protocols (bowties/hourglasses)  in LEC systems that have significant consequences on achievable performance.

\paragraph{Success stories} Arguably the most complete body of theory and algorithms in learning-enabled control is in the context of linear systems, in particular in the context of LQR control. Initiated by \cite{abbasi2011regret} and repopularized in 
\cite{Dean2018, Dean2019a}, follow up work has shown that a layered approach of system-identification followed by certainty-equivalent control is optimal for LQR \cite{mania2019certainty}, that model-based RL is more data-efficient \cite{tu2019gap, kaiser2019model, polydoros2017survey} than model-free (end-to-end) approaches, more naturally allows for robustness/safety \cite{Dean2019b}, and that layered approaches naturally allow extensions to distributed settings \cite{fattahi2019efficient,qu2020scalable}.  If and how these concepts extend to the general nonlinear setting remains an open question, and exciting opportunity for architectural thinking to have significant impact both within and beyond the (learning-enabled) controls community.

Indeed, exciting first steps, again implicitly aimed at achieving DeSS that balance the adaptibility/performane of RL with the safety/robustness of control-based methods, have emerged in recent years.  For example, Lyapunov/Barrier constraints have been used as safety shields in RL \cite{chow2018lyapunov, taylor2020learning, perkins2002lyapunov,rodriguez2022lyanet}, and priors/regularizers rooted in model-based robust control \cite{cheng2019control, johannink2019residual} have been used to bias model-free RL methods towards solutions with desirable properties.  We see once again a common theme emerging: both the machine learning and controls communities are converging towards methods that explore intermediate architectures, in an attempt to achieve DeSS in the face of hard limits, in this case by appropriately integrating model-based, model-free, control theoretic, and data-driven techniques.
\end{sidebar}

==> tex-files/learning-vignette.tex <==
Previous sections in this document highlight the important, if not ad-hoc, role that architecture plays in the context of Learning-Enabled Control (LEC).  Sections \ref{sec:Robotics-And-Automation}, \ref{sec:Learning-Data-Driven-Control}, \ref{sec:safety}, and \ref{sec:resilience} all implicitly or explicitly reference the importance of correctly integrating traditional and learning-based control methods to co-optimize various metrics, such as speed, sample-complexity, safety, security, robustness, adaptation and performance.  In this subsection, we highlight how much of the aforementioned discussion can be viewed through the lens of the key concepts of DCA, namely levels, laws, DeSS, and layering.  To ground our discussion, we introduce the following concrete motivational example.

\paragraph{Motivating example}
Consider two future autonomous system use-cases: (i) a bomb defusing rover sent into an unfamiliar, GPS and communication denied environment (e.g., a cave or mine), tasked with the objective of locating and defusing an improvised explosive device, and (ii) an autonomous racing drone competing in a future autonomous incarnation of the \href{https://thedroneracingleague.com/}{Drone Racing League}, akin to the \href{https://www.herox.com/alphapilot/community}{AlphaPilot} competition \cite{foehn2020alphapilot}.  Both systems will make decisions %using on-board autonomy that must infer and predict the system and world state 
based on inputs from a combination of simple, single output sensing devices, such as inertial measurement units, and complex, high dimensional output sensing modalities, such as cameras and LIDAR.  What does this shift from systems relying only on simple, single output sensing devices to systems that incorporate rich, complex perceptual sensing modalities mean for how we design safety-critical autonomous systems?  Conversely, given the inextricable role that machine and deep learning play in designing modern perceptual sensors and predictors, do current methods and best-practices in these fields result in perceptual sensors that are well suited for use within safety-critical control loops?

%- we refer to this map from complex sensory inputs to decision and control as the \emph{perception/action pipeline}, and it is the focus of this proposal.

\sdbarfig{\includegraphics[width=\columnwidth]{architecture/cartoon-tradeoff-sec1.pdf}}
{Perceptual sensors may have very different robustness \& performance requirements depending on dynamics, environments, objectives, and constraints.\label{fig:cartoon-tradeoff}}

Note however, that our two motivating examples raise an even more fundamental question: given the vastly different dynamics, environments, objectives, and safety risks/constraints, should these two systems have perceptual sensors with different properties?  Indeed, due to the \emph{extremely} safety critical nature of the bomb defusing task, an emphasis on robustness, risk aversion, and safety seems necessary.  Conversely, the designer of the drone racer may be willing to sacrifice robustness to maximize responsiveness and lower lap-time.  This extreme diversity in requirements, conceptually illustrated in Fig.~\ref{fig:cartoon-tradeoff}, highlights the need for a principled approach to navigate tradeoffs in this complex design space.  More specifically, this case-study makes a clear case for identifying fundamental speed-accuracy (peformance-robustness) tradeoffs and for designing layered-architectures that achieve a desired DeSS point on the resulting Pareto surface.  In this context, the diversity component of DeSS is provided by the balance between hardware and software, as well as traditional and learning-enabled control.

With this architectural framing in mind, consider two philosophically opposed approaches to designing suitable perception/action pipelines: (i) layered, and (ii) end-to-end \cite{bojarski2016end,pomerleau1989alvinn,levine2016end} approaches. The familiar layered (or modular) approach, rooted in engineering best-practices, designs different layers (perception, prediction, localization, planning, control) independently, and interconnects them via pre-specified (rigid) protocols. While the benefits of such approaches are well known to the controls community, and are also well suited to large organizational structures, this approach limits interaction between layers to often ad-hoc specifications shared between teams, thus limiting end-to-end optimization \cite{zeng2019end}.  
The end-to-end approach, classically favored by the deep reinforcement learning community, in contrast seeks to learn an optimized map directly from pixels (or other high-dimensional sensory inputs) to actions.  While such approaches have the advantage of optimizing the full perception/action pipeline for a specific application, and have led to impressive demonstrations, the resulting systems are opaque, difficult to troubleshoot, and lack safety guarantees.  Further, they often preclude prior knowledge from being incorporated into learning/design, leading to increased sample complexity and brittle algorithms.
\end{sidebar}

\begin{sidebar}{\continuesidebar}

\paragraph{The LEC Architecture Design Space} These two approaches can be viewed as extreme points of a broader architectural design space, with the layered approach optimizing for interpretability, modularity, and (arguably) safety/robustness, and the end-to-end approach optimizing for performance and simplicity (of implementation).  A coherent theory of architecture will allow for a principled exploration of the entire design-space.  Indeed, existing work in the robotics and machine learning community, in particular in the context of safety-critical applications such as autonomous vehicles (AV), have recognized the need for diversity enabled architectures.  For example, the robotics community has recently begun to explore similar questions to those raised in this section, seeking to shift to an intermediate design philosophy. In the AV community, \cite{zeng2019end,liang2020pnpnet,luo2018fast,sauer2018conditional,williams2018information} propose end-to-end learnable motion planners, that take as input raw perceptual data (e.g, pixels or LIDAR), and produce both interpretable intermediate representations in the form of 3D detections and a space-time cost volume that is optimized via sampling by the planner.  In the context of agile perception based flight, recent work \cite{kaufmann2018deep} combines a CNN for perceptual sensing, which maps raw images to waypoints and desired speeds, which are then used by a planning module to generate short trajectory segments and corresponding motor commands to reach the desired goal. 

These preliminary results highlight two important points. First, that two independent sub-communities within robotics have converged to and discovered similar design pipelines highlights both the importance of architectural choices in LEC design, and the \emph{need for a unified underlying theoretical and algorithmic framework} for making these design choices.  Second, the \emph{level at which representations are shared between perception and action components is an important design decision}: indeed, as described in \cite{kaufmann2018deep}, sharing discrete navigation commands as in \cite{kim2015deep,loquercio2018dronet} improves robustness at the expense of performance, and conversely, representations at the level of direct control \cite{kahn2017plato} can lead to highly agile control at the expense of high sample complexity and system fragility.  These are concrete examples of designed interfaces/protocols (bowties/hourglasses)  in LEC systems that have significant consequences on achievable performance.



\paragraph{Success stories} Arguably the most complete body of theory and algorithms in LEC is in the context of linear systems, in particular in the context of LQR control. Initiated by \cite{abbasi2011regret} and repopularized in 
\cite{Dean2018, Dean2019a}, follow up work has shown that a layered approach of a system-identification component followed by certainty-equivalent optimal controller is optimal for LQR \cite{mania2019certainty}, that model-based RL is more data-efficient \cite{tu2019gap, kaiser2019model, polydoros2017survey} than model-free (end-to-end) approaches, and more naturally allows for robustness/safety \cite{ Dean2019b}, and that layered approaches naturally allow extensions to distributed settings \cite{fattahi2019efficient,qu2020scalable}.  If and how these concepts extend to the general nonlinear setting remains an open question, and an exciting opportunity for architectural thinking to have significant impact both within and beyond the (learning-enabled) controls community.

Indeed, exciting first steps, again implicitly aimed at achieving DeSS that balance the adaptibility/performance of RL with the safety/robustness of control-based methods, have emerged in recent years.  For example, Lyapunov/Barrier constraints (introduced in \S\ref{sec:safety}) have been used as safety shields in RL \cite{chow2018lyapunov, taylor2020learning, perkins2002lyapunov}, and priors/regularizers rooted in model-based robust control \cite{cheng2019control, johannink2019residual} have been used to bias model-free RL methods towards solutions with desirable properties.  We see once again a common theme emerging: both the machine learning and controls communities are converging towards methods that explore intermediate architectures, in an attempt to achieve DeSS in the face of hard limits, in this case by appropriately integrating model-based, model-free, control theoretic, and data-driven techniques.

\end{sidebar}

\begin{sidebar}{\continuesidebar}

\paragraph{New directions}
In addition to the questions raised above, we comment here on two complementary directions that do not fit within the current framework, but need to be addressed within any successful theory of architecture for LEC systems.
\begin{itemize}
    \item \emph{Architecture as inductive bias:} The term architecture has a specific meaning within the deep-learning community.  In particular, it denotes design choices in the function to be learned itself, most often to reflect prior knowledge of the downstream task (i.e., to impose inductive biases in the learning task).  A familiar example is the use of Convolutional Neural Networks (CNNs) in vision-based tasks, to encode that the learned map should enjoy translational equivariance/invariance.  The idea of architecture as inductive bias has recently been placed on firm theoretical footing by viewing it through the lens of geometric deep learning \cite{bronstein2017geometric}, which seeks to formalize the mapping from underlying symmetries in the data to the architectural design choices of a neural network.  An exciting and important question for the controls community is to identify novel architectures that enforce symmetries arising from dynamical systems and feedback control, see \cite{allen2020lagnetvip} for an exciting first step in this direction.
    \item \emph{Adversarial learning-enabled control:} The machine learning community's most formal attempt at navigating robustness/accuracy accuracy tradeoffs can be found in the adversarial learning literature.  This body of work has analyzed performance-robustness tradeoffs in adversarially robust learning, including precise characterizations of the generalization errors of standard versus adversarially trained models under various theoretical models \citep{zhang2019theoretically,javanmard2020precise, hassani2022curse}, and ``no free lunch'' theorems for obtaining adversarially robust models \citep{tsipras2018robustness, dohmatob2019generalized, yin2019rademacher}.  The successful characterization of such performance-robustness tradeoffs in machine learning motivates studying similar tradeoffs in the context of LEC systems. However, the theoretical results from this area are largely intended for the supervised learning setting and do not immediately apply to data generated by dynamical systems. The extension of adversarial robustness results in machine learning to various control problems is an exciting and active area of research \citep{al2020accuracy, lee2021adversarial, zhang2021adversarially, havens2022revisiting}, which is explicitly aimed at identifying DeSS by balancing performance with robustness.
\end{itemize}

\paragraph{Final thoughts} 
We believe that our discussion makes clear that a new, unified way of thinking about learning and control is needed that actively and explicitly reasons about how learning-enabled and traditional control components are integrated, interconnected, and interfaced.  Given the maturity of both control theory and machine learning as independent disciplines, we argue that architectural questions lie at the core of current challenges in LEC.  This makes adding rigor and structure to what is currently an ad-hoc architectural design process all the more imperative and exciting.

==> tex-files/neuro-vignette.tex <==
\sdbarinitial{L}ayered architectures and DeSS have been studied for decades in engineering  \cite{ChiangEtAl2007} and (systems) biology \cite{csete2002reverse} but are relatively new to neuroscience.
In \cite{Wang2019TAC, Nakahira2021, Paper1, Paper3} we approach sensorimotor control as a control architecture.  We start with a 'simple' problem from neuroscience introduced in \cite{ND15} and developed further in \cite{Nakahira2021}, to illustrate the concepts necessary to understand DeSS. While prior work includes information theory constraints (e.g. channel capacity) in sensorimotor control (e.g. \cite{Martins2007}),  \cite{Nakahira2021} is the first work that considers both bandwidth/quantization and delay (delay is especially important in control applications). 

Sensorimotor control was studied in the context of the multisensory task of mountain bike riding using a video game as the experimental platform \cite{Nakahira2021}. The game captures tunable requirements on player performance which, together with speed-accuracy tradeoffs (SATs) in sensor and actuator level components, require layered architectures in the nervous system to create diversity-enabled sweet spots (DeSS, Fig. (\ref{fig:ynfig}) \cite{Nakahira2021, Nakahira2019b}.  \textbf{This could be cut.}See Fig. SS

Fig.~\ref{fig:ynfig} is a simple cartoon that highlights layers, and motivates levels, SATs, and DeSS as discussed below. 

	
	




Naively, success in the biking task seems to require speed and accuracy that the raw hardware lacks, making non-layered solutions infeasible. The layered nervous system breaks the overall biking problem into a high \textit{trails} layer of slow but accurate vision with trail look-ahead for advanced warning, and a low \textit{bumps} layer that uses fast but inaccurate muscle spindles and proprioception to sense and reject bump disturbances. 
%The motor commands from these two control loops to the muscles simply add in the optimal case, as well as in experiments \cite{Nakahira2021,Liu2019}, though muscles have their own SATs as demonstrated by Fitts Law (\cite{Fitts}). 

Effective architectures (such as layering) create a DeSS where diverse hardware enables a sweet spot that is both fast and accurate even though no parts are. In other words this simple model captures the most fundamental benefit of universal architectures, creation of a \textit{DeSS} in function at the system \textit{level} that the components alone cannot provide. This requires understanding \textit{laws} at the component level and their impact on the system level, and how \textit{layers} achieve a DeSS that obeys all laws. An additional crucial feature of complex control systems is internal delays, which must be considered in the context of control architecture of large societal systems.

\sdbarfig{\includegraphics[width=19.0pc]{architecture/layered_yorie_ctrller.png}}{Layered controller adapted from a model of mountain biking \cite{Nakahira2021} that illustrate diversity-enabled sweet spots (DeSS). This controller optimally layers diverse  components from axons to muscle that have severe speed-accuracy tradeoffs (SATs) to produce optimal behavior with good speed \textit{and} accuracy in both theory and extensive experiments. The optimal high layer controller (H) uses delayed sensing (vision) with high accuracy, while the optimal lower layer (L) uses less accurate sensors with smaller delays.  The optimal controller is a simple combination of the separately optimal H and L, only possible because humans multiplex these tasks well.  See the text and \cite{Nakahira2021} for further details.\label{fig:ynfig}}

 
In theory, internal delays and other such constraints (sparsity, locality, quantization) made controller synthesis intractable \cite{Witsenhausen1968}, and speed of light electronics made the practical need negligible.  But existing bio and neuro and future tech and social control systems have significant internal constraints, and we need and have a substantial theory upgrade in System Level Synthesis (SLS) \cite{Anderson2019, Wang2019TAC} to address them.  SLS is essential in scaling to more general problems.

